Discovering Interesting Plots in Production Yield Data Analytics

An analytic process is iterative between two agents, an analyst and an analytic toolbox. Each iteration comprises three main steps: preparing a dataset, running an analytic tool, and evaluating the result, where dataset preparation and result evaluation, conducted by the analyst, are largely domain-knowledge driven. In this work, the focus is on automating the result evaluation step. The underlying problem is to identify plots that are deemed interesting by an analyst. We propose a methodology to learn such analyst's intent based on Generative Adversarial Networks (GANs) and demonstrate its applications in the context of production yield optimization using data collected from several product lines.

==> bib.tex <==
\begin{thebibliography}{1}

\itemsep=0pt
\topsep = 0pt
\partopsep=0pt
\itemsep= 0cm
\parsep=0pt
\parskip= 0cm

\vspace{-0.4cm}

\small 

\bibitem{AEC2011}
Guidelines for Part Average Testing.
\newblock{Automotive Electronic Council}, AEC-Q001 Rev-D, December 9, 2011.

\bibitem{freescale}
Manuel J. Moreno-Lizaranzu and Federico Cuesta.
\newblock{Improving Electronic Sensor Reliability by Robust
Outlier Screening}.
{\it Sensors} 2013, 13, pp. 13521--13542

\bibitem{ken2006}
Ken Butler, et. al.
\newblock{Successful Development and Implementation of Statistical
Outlier Techniques on 90nm and 65nm process driver devices}
IEEE {\it IRPS}, 2006, pp. 552--559.

\bibitem{NNR2000}
W. R. Daasch, J. McNames, D. Bockelman, K. Cota,
R. Madge.
\newblock{Variance Reduction Using Wafer Patterns
in IDDQ Data}.
International Test Conference, Oct 2000, pp. 189--198.
%%% This is the NNR paper Nearest Neighbor Residuals

\bibitem{LA2001}
R. Daasch, K. Cota, J. McNames, and R. Madge.
\newblock{Neighbor Selection for Variance Reduction in IDDQ
and Other Parametric Data}.
IEEE ITC, Oct 2001, pp. 92--100.
%%% Location Averaging (LA)

%\bibitem{PCA2005}
%A. Nahar, R. Daasch, and S. Subramaniam.
%\newblock{Burn-in Reduction Using Principle Component Analysis}.
%ITC, 2005, Paper 7.2.
%%%% Principle Component Analysis (PCA)

%\bibitem{PCA2008}
%Peter M. O'Neill. 
%\newblock{Production Multivariate Outlier Detection
%Using Principal Components.} IEEE ITC, 2008.

%\bibitem{ITC2012}
%Nik Sumikawa, Jeff Tikkanen, Li-C. Wang,
%LeRoy Winemberg and Magdy S. Abadir.
%\newblock{Screening Customer Returns With Multivariate Test Analysis}. 
%ITC, 2012.


\bibitem{OL}
Charu C. Aggarwal.
\newblock{Outlier Analysis}. 
Springer, 2013. 

\bibitem{NFL}
David Wolpert.
\newblock{The Lack of A Priori Distinctions between Learning Algorithms}. 
{\em Neural Computation}, 1996, pp. 1341-1390.

\bibitem{DE}
B.W. Silverman.
\newblock{Density Estimation for Statistics and Data Analysis}.
Monographs on Stat. and App. Prob.,  v26, 1986.

\bibitem{DEI}
Jan Beirlant and Luc Devroye.
\newblock{On the impossibility of estimating densities in the extreme tail}.
{\em Statistics \& Probability Letters}, 43, 1999, pp. 57-64. 

%\bibitem{SVM}
%Vapnik, Vladimir, and Sayan Mukherjee. 
%\newblock{Support Vector Method for Multivariate Density Estimation}. 
%In {\it NIPS}, 1999, pp. 659-665. 

\bibitem{ITC2015}
Sebastian Siatkowski, et al.
\newblock{Generalization of an outlier model into a ``global'' perspective}. 
ITC, 2015.

\bibitem{vts16}
Sebastian Siatkowski, at el.
\newblock{Consistency in wafer based outlier screening}
IEEE VLSI Test Symposium, 2016. 

\bibitem{Grubbs}
F. Grubbs. 
\newblock{Procedures for detecting outlying observations in samples}. 
\newblock{\it Technometrics} 11, 1969, pp. 1-–21.

%\bibitem{Johnson}
%F. Hernandez and R. A. Johnson.
%\newblock{The large-sample behavior of transformations to normality}. 
%Journal of American Statistical Association, v75, no 372, 1980, pp. 855--861.

%\bibitem{Normal}
%Y-M. Chou, Alan M. Polansky, Robert L. Mason. 
%\newblock{Transforming non-normal data to normality in statistical process control}. 
%Journal of Quality Technolology, v30, no 2, 1998, pp. 133–-141.

\bibitem{KS}
Eric Jones, Travis Oliphant, Pearu Peterson, and others.
\newblock{{SciPy}: Open source scientific tools for {Python}},
http://www.scipy.org/, 2001-. 

\bibitem{Mah}
Scikit-learn: Machine Learning in Python, Pedregosa et al., JMLR 12, 2011, pp. 2825-2830. 
%(http://scikit-learn.org/stable/modules/covariance.html)


\end{thebibliography}


